A UNet Model for Accelerated Preprocessing of CRISM Hyperspectral Data for Mineral Identification on Mars

Accurate mineral identification on the Martian surface is critical for understanding the planet's geological history. This paper presents a UNet-based autoencoder model for efficient spectral preprocessing of CRISM MTRDR hyperspectral data, addressing the limitations of traditional methods that are computationally intensive and time-consuming. The proposed model automates key preprocessing steps, such as smoothing and continuum removal, while preserving essential mineral absorption features. Trained on augmented spectra from the MICA spectral library, the model introduces realistic variability to simulate MTRDR data conditions. By integrating this framework, preprocessing time for an 800x800 MTRDR scene is reduced from 1.5 hours to just 5 minutes on an NVIDIA T1600 GPU. The preprocessed spectra are subsequently classified using MICAnet, a deep learning model for Martian mineral identification. Evaluation on labeled CRISM TRDR data demonstrates that the proposed approach achieves competitive accuracy while significantly enhancing preprocessing efficiency. This work highlights the potential of the UNet-based preprocessing framework to improve the speed and reliability of mineral mapping on Mars.

==> architecture1.tex <==
The proposed model is a 1D-UNet designed to process hyperspectral data from the CRISM MTRDR dataset. This architecture is specialized for spectral data, where each input spectrum comprises 240 bands, corresponding to the selected wavelength range between $1$ to $2.6$ micrometers. The model consists of an encoder-decoder structure with skip connections, enabling feature extraction at multiple resolutions while preserving essential spectral information through skip connections. 

Let $\mathbf{X} \in \mathbb{R}^{240 \times 1}$ represent the input spectrum, where $240$ is the number of spectral bands for each pixel. The network outputs a processed spectrum of the same dimensions. The main components of the architecture are detailed below.

\subsection*{Encoder Blocks}

Each encoder block is designed to progressively reduce the spectral dimensionality while extracting important features. Let $f_i$ denote the feature maps for the $i^{\text{th}}$ encoder block.

The $i^{\text{th}}$ encoder block consists of:
\begin{enumerate}
    \item \textbf{First convolutional layer:} A convolution operation with stride $1$ to preserve the spatial resolution while expanding the feature dimension. Mathematically, for input $\mathbf{X}_{i-1}$ to the block, we have:
    \[
    \mathbf{Z}_{i,1} = \sigma\left(\mathbf{W}_{i,1} * \mathbf{X}_{i-1} + \mathbf{b}_{i,1}\right),
    \]
    where $\mathbf{W}_{i,1}$ and $\mathbf{b}_{i,1}$ are the weights and biases of the first convolution, $\sigma$ is the activation function (ReLU), and $*$ denotes convolution.

    \item \textbf{Second convolutional layer:} A convolution with stride $2$, reducing the spectral dimensionality by half to capture high-level features. This yields:
    \[
    \mathbf{f}_{i} = \sigma\left(\mathbf{W}_{i,2} * \mathbf{Z}_{i,1} + \mathbf{b}_{i,2}\right).
    \]
\end{enumerate}

The output $\mathbf{f}_{i}$ from each encoder block is passed to both the next encoder block and the corresponding decoder block through a skip connection.

\subsection*{Decoder Blocks}

The decoder blocks reconstruct the spectrum by upsampling and refining features from the encoder. Let $\mathbf{f}_{i}^d$ denote the features in the $i^{\text{th}}$ decoder block.

Each decoder block consists of:
\begin{enumerate}
    \item \textbf{Upsampling layer:} This layer doubles the input dimensionality by applying a convolution transpose operation with stride $2$, generating an upsampled representation $\mathbf{U}_{i}$:
    \[
    \mathbf{U}_{i} = \sigma\left(\mathbf{W}_{i}^{\text{up}} * \mathbf{f}_{i+1}^d + \mathbf{b}_{i}^{\text{up}}\right).
    \]

    \item \textbf{Concatenation with skip connection:} The upsampled output $\mathbf{U}_{i}$ is concatenated with the output from the corresponding encoder block, $\mathbf{f}_{i}$, to retain high-resolution features:
    \[
    \mathbf{V}_{i} = \text{concat}\left(\mathbf{U}_{i}, \mathbf{f}_{i}\right).
    \]

    \item \textbf{Two convolutional layers:} The concatenated output $\mathbf{V}_{i}$ is passed through two convolutional layers with stride $1$ to refine the spectral features. For the first convolution:
    \[
    \mathbf{Z}_{i,1}^d = \sigma\left(\mathbf{W}_{i,1}^d * \mathbf{V}_{i} + \mathbf{b}_{i,1}^d\right),
    \]
    and for the second convolution:
    \[
    \mathbf{f}_{i}^d = \sigma\left(\mathbf{W}_{i,2}^d * \mathbf{Z}_{i,1}^d + \mathbf{b}_{i,2}^d\right).
    \]
\end{enumerate}

\subsection*{Input and Output Layers}

The model begins with an \textbf{input layer} that accepts the 1D spectral data $\mathbf{X} \in \mathbb{R}^{240 \times 1}$. After the final decoder block, an \textbf{output layer} with the same shape as the input layer produces the processed spectrum $\mathbf{Y} \in \mathbb{R}^{240 \times 1}$:
\[
\mathbf{Y} = \sigma\left(\mathbf{W}_{\text{out}} * \mathbf{f}_{1}^d + \mathbf{b}_{\text{out}}\right),
\]
where $\mathbf{W}_{\text{out}}$ and $\mathbf{b}_{\text{out}}$ are the parameters of the final convolutional layer.

The encoder-decoder structure with skip connections is designed to capture both high- and low-level spectral features, enhancing the distinguishable absorption signatures required for mineral identification. By incorporating downsampling and upsampling layers with appropriate strides, the model efficiently compresses and reconstructs the spectral data. This design enables both dimensionality reduction and the retention of critical absorption features across the 240 spectral bands, offering an efficient alternative to conventional preprocessing steps.

==> architecture2.tex <==
The proposed model is a 1D-UNet architecture adapted to process hyperspectral data. Each pixel spectrum in the CRISM MTRDR dataset consists of 240 bands, corresponding to specific wavelengths in the range of approximately 1 to 2.6 micrometers. This 1D-UNet model integrates convolutional layers, encoder and decoder blocks, skip connections, and a bottleneck block to efficiently process spectral data, reducing the need for traditional preprocessing steps.

\subsection{Input Layer}

Let the input spectrum for each pixel be represented as:
\begin{equation}
X = [x_1, x_2, \dots, x_{240}]
\end{equation}
where $X \in \mathbb{R}^{240}$ represents the spectral bands.

\subsection{Encoder Blocks}

Each encoder block consists of two convolutional layers. Let $L_i$ denote the $i$-th encoder block in the network. The encoder operation within each block is defined as:
\begin{equation}
L_i = \text{Conv1D}(L_{i-1}, k_i, s=1) \rightarrow \text{BatchNorm} \rightarrow \text{ReLU}
\end{equation}
where $\text{Conv1D}$ is a 1D convolution operation with kernel size $k_i$, stride $s=1$, followed by batch normalization and a ReLU activation function. To reduce dimensionality, the second convolution in each encoder block has a stride of $s=2$:
\begin{equation}
L_i = \text{Conv1D}(L_i, k_i, s=2) \rightarrow \text{BatchNorm} \rightarrow \text{ReLU}
\end{equation}

This structure allows the model to capture hierarchical spectral features while downsampling the input, which reduces the spatial dimensions and retains crucial spectral information.

\subsection{Bottleneck Block}

The bottleneck block connects the encoder and decoder sections and further processes the compressed spectral information. It contains two convolutional layers. The first layer operates with a stride of $s=1$ and the second with a stride of $s=2$:
\begin{equation}
L_{\text{bottleneck}} = \text{Conv1D}(L_{\text{encoder\_last}}, k, s=1) \rightarrow \text{BatchNorm} \rightarrow \text{ReLU} \rightarrow \text{Conv1D}(L_{\text{encoder\_last}}, k, s=2) \rightarrow \text{BatchNorm} \rightarrow \text{ReLU} \rightarrow \text{Upsample}(s=2)
\end{equation}
where $\text{Upsample}(s=2)$ upsamples the feature dimensions to prepare for decoding. This block captures the most compressed features, serving as the primary feature extraction layer.

\subsection{Decoder Blocks}

Each decoder block reconstructs the original input dimensions using upsampling and convolutional operations. The decoder block $D_i$ is given by:
\begin{equation}
D_i = \text{Upsample}(L_{D_{i-1}}, s=2) \rightarrow \text{Conv1D}(k, s=1) \rightarrow \text{BatchNorm} \rightarrow \text{ReLU}
\end{equation}
This operation is followed by two convolutional layers with stride $s=1$, preserving spatial information as the data dimensions increase:
\begin{equation}
D_i = \text{Conv1D}(D_i, k, s=1) \rightarrow \text{BatchNorm} \rightarrow \text{ReLU}
\end{equation}

\subsection{Skip Connections}

Skip connections are added between each encoder block $L_i$ and the corresponding decoder block $D_i$. These connections allow the model to retain high-resolution spectral features from earlier layers, preventing information loss:
\begin{equation}
D_i = D_i + L_i
\end{equation}

\subsection{Output Layer}

The output layer has the same dimensionality as the input, representing the preprocessed spectrum for each pixel:
\begin{equation}
\hat{X} = [\hat{x}_1, \hat{x}_2, \dots, \hat{x}_{240}]
\end{equation}

The choice of using 1D convolutions and encoder-decoder architecture enables efficient processing of spectral data by leveraging hierarchical feature extraction and dimensionality reduction. By integrating batch normalization and skip connections, the model maintains stability during training, speeds up convergence, and preserves essential spectral details. The stride-2 convolutions in the encoder blocks and the upsampling layers in the decoder blocks contribute to computational efficiency, making the model suitable for real-time data preprocessing. This model structure is further fine-tuned in an ablation study to determine the optimal configuration of encoder and decoder blocks.

The final preprocessed output $\hat{X}$ can be directly fed into downstream mineral classification models, significantly reducing the computation time compared to traditional preprocessing pipelines.


==> architecture_edited.tex <==
The proposed model is a 1D-UNet designed to process hyperspectral data from the CRISM MTRDR dataset. This architecture is specialized for spectral data, where each input spectrum comprises 240 bands, corresponding to the selected wavelength range between $1$ to $2.6$ micrometers. The model consists of an encoder-decoder structure with skip connections, enabling feature extraction at multiple resolutions while preserving essential spectral information through skip connections. 

Let $\mathbf{X} \in \mathbb{R}^{240 \times 1}$ represent the input spectrum, where $240$ is the number of spectral bands for each pixel. The network outputs a processed spectrum of the same dimensions. The main components of the architecture are detailed below.


\subsection*{Input Layer}

Let the input spectrum for each pixel be represented as:
\begin{equation}
\mathbf{X} = [x_1, x_2, \dots, x_{240}]
\end{equation}
where $\mathbf{X} \in \mathbb{R}^{240}$ represents the spectral bands.

\subsection*{Encoder Blocks}

Each encoder block is designed to progressively reduce the spectral dimensionality while extracting important features. Let $f_i$ denote the feature maps for the $i^{\text{th}}$ encoder block.

The $i^{\text{th}}$ encoder block consists of:
\begin{enumerate}
    \item \textbf{First convolutional layer:} A convolution operation with stride $1$ to preserve the spatial resolution while expanding the feature dimension. Mathematically, for input $\mathbf{X}_{i-1}$ to the block, we have:
    \begin{equation}
    \mathbf{Z}_{i,1} = \sigma\left(\mathbf{W}_{i,1} * \mathbf{X}_{i-1} + \mathbf{b}_{i,1}\right),
    \end{equation}
    where $\mathbf{W}_{i,1}$ and $\mathbf{b}_{i,1}$ are the weights and biases of the first convolution, $\sigma$ is the activation function (ReLU), and $*$ denotes convolution.

    \item \textbf{Second convolutional layer:} A convolution with stride $2$, reducing the spectral dimensionality by half to capture high-level features. This yields:
    \begin{equation}
    \mathbf{f}_{i} = \sigma\left(\mathbf{W}_{i,2} * \mathbf{Z}_{i,1} + \mathbf{b}_{i,2}\right).
    \end{equation}
\end{enumerate}

The output $\mathbf{f}_{i}$ from each encoder block is passed to both the next encoder block and the corresponding decoder block through a skip connection.

\subsection*{Bottleneck Block}

The bottleneck block connects the encoder and decoder sections and further processes the compressed spectral information. It contains two convolutional layers and one upsample layer. The first convolution layer operates with a stride of $s=1$, whereas the second convolution layer and the upsample layer operate with stride of $s=2$. The upsample layer upsamples the feature dimensions to prepare for decoding. This block captures the most compressed features, serving as the primary feature extraction layer.
\begin{equation}
L_{\text{B,1}} = \sigma(\sigma(\sigma()))
\end{equation}
\begin{equation}
L_{\text{B,2}} = \sigma(\sigma(\sigma()))
\end{equation}
\begin{equation}
L_{\text{B,3}} = \sigma(\sigma(\sigma()))
\end{equation}
where 
\begin{equation}
    \text{Conv1D}(L_{\text{encoder\_last}}, k, s=1) \rightarrow \text{Conv1D}(L_{\text{encoder\_last}}, k, s=2) \rightarrow \text{Upsample}(s=2)
\end{equation}
\subsection*{Decoder Blocks}

The decoder blocks reconstruct the spectrum by upsampling and refining features from the encoder. Let $\mathbf{f}_{i}^d$ denote the features in the $i^{\text{th}}$ decoder block.

Each decoder block consists of:
\begin{enumerate}
    \item \textbf{Upsampling layer:} This layer doubles the input dimensionality by applying a convolution transpose operation with stride $2$, generating an upsampled representation $\mathbf{U}_{i}$:
    \begin{equation}
    \mathbf{U}_{i} = \sigma\left(\mathbf{W}_{i}^{\text{up}} * \mathbf{f}_{i+1}^d + \mathbf{b}_{i}^{\text{up}}\right).
    \end{equation}

    \item \textbf{Concatenation with skip connection:} The upsampled output $\mathbf{U}_{i}$ is concatenated with the output from the corresponding encoder block, $\mathbf{f}_{i}$, to retain high-resolution features:
    \begin{equation}
    \mathbf{V}_{i} = \text{concat}\left(\mathbf{U}_{i}, \mathbf{f}_{i}\right).
    \end{equation}

    \item \textbf{Two convolutional layers:} The concatenated output $\mathbf{V}_{i}$ is passed through two convolutional layers with stride $1$ to refine the spectral features. For the first convolution:
    \begin{equation}
    \mathbf{Z}_{i,1}^d = \sigma\left(\mathbf{W}_{i,1}^d * \mathbf{V}_{i} + \mathbf{b}_{i,1}^d\right),
    \end{equation}
    and for the second convolution:
    \begin{equation}
    \mathbf{f}_{i}^d = \sigma\left(\mathbf{W}_{i,2}^d * \mathbf{Z}_{i,1}^d + \mathbf{b}_{i,2}^d\right).
    \end{equation}
\end{enumerate}

\subsection*{Output Layer}

After the final decoder block, an \textbf{output layer} with the same shape as the input layer produces the processed spectrum $\hat{\mathbf{X}} \in \mathbb{R}^{240 \times 1}$:
\begin{equation}
\hat{\mathbf{X}} = \sigma\left(\mathbf{W}_{\text{out}} * \mathbf{f}_{1}^d + \mathbf{b}_{\text{out}}\right),
\end{equation}
where $\mathbf{W}_{\text{out}}$ and $\mathbf{b}_{\text{out}}$ are the parameters of the final convolutional layer.

Each of the convolution layers are followed by batch normalization layers and each of the convolution and upsamplimg layers are equipped with ReLU activation function.
The choice of using 1D convolutions and encoder-decoder architecture enables efficient processing of spectral data by leveraging hierarchical feature extraction and dimensionality reduction. By integrating batch normalization and skip connections, the model maintains stability during training, speeds up convergence, and preserves essential spectral details. The stride-2 convolutions in the encoder blocks and the upsampling layers in the decoder blocks contribute to computational efficiency, making the model suitable for real-time data preprocessing. This model structure is further fine-tuned in an ablation study to determine the optimal configuration of encoder and decoder blocks.

The final preprocessed output $\hat{X}$ can be directly fed into downstream mineral classification models, significantly reducing the computation time compared to traditional preprocessing pipelines.

==> introduction.tex <==
Mineral identification on the Martian surface is crucial for understanding the planet's geological history, assessing its potential for past habitability, and identifying resources that may support future exploration or even potential colonization. The Compact Reconnaissance Imaging Spectrometer for Mars (CRISM) sensor on the Mars Reconnaissance Orbiter captures hyperspectral data across visible and infrared wavelengths, enabling a detailed analysis of Martian surface composition. After atmospheric and photometric corrections, CRISM generates data products, such as the Map-Projected Targeted Reduced Data Record (MTRDR), which contain spectral information with a resolution of approximately 6 nm. This high-resolution data provides distinguishable spectral signatures of various minerals, which are crucial for accurate mineral identification on Mars.

Numerous methods have been applied in the literature to identify minerals on the Martian surface using hyperspectral data. Supervised techniques, such as Support Vector Machines (SVM), Random Forests (RF), and Convolutional Neural Networks (CNNs), and unsupervised approaches like k-means clustering have shown promise in this area. These methods leverage spectral features unique to certain minerals, enabling effective classification. However, before performing mineral identification, it is essential to preprocess the Martian spectra to minimize noise, adjust spectral baselines, and enhance the distinguishable spectral absorption features. Preprocessing is critical for optimizing the quality and reliability of mineral classification and ensuring that the inherent mineralogical information is accurately represented.

Several preprocessing steps have been identified as crucial in preparing Martian spectral data. Key steps include spike removal, smoothing, wavelength range selection, scaling, and continuum removal. Smoothing addresses fluctuation noise and random spikes that can distort spectral data. Meanwhile, continuum removal normalizes the baseline curvature caused by mixed spectra in real MTRDR data, thus enhancing the clarity of absorption features and allowing models to distinguish mineral signatures more effectively. These preprocessing steps have proven essential for increasing the accuracy and reliability of mineral classification, and their application forms a preprocessing pipeline that is commonly used to prepare hyperspectral data for subsequent analysis.

While these preprocessing operations can be computed in linear time, they are not linear transformations. Each step depends on the spectral features themselves, making the processing of large-scale MTRDR hyperspectral images a time-consuming task. For instance, a single MTRDR scene of 800 × 800 pixels containing around 70% informative pixels may take up to 1.5 hours to preprocess on a standard Intel i7-9300H processor with 8 GB of RAM. This significant computational demand presents a barrier to efficient mineral mapping across the planet, especially as the scale of Martian data acquisition continues to grow.

In this paper, we propose a neural network model based on the UNet architecture to streamline this preprocessing pipeline. The UNet model, typically used for image segmentation, is adapted here for 1D convolution to process hyperspectral spectral data more efficiently. By integrating spike removal, smoothing, wavelength range standardization, scaling, and continuum removal within a single model, the proposed approach bypasses the need for a separate preprocessing pipeline. The model directly enhances the spectral clarity of raw data from the MTRDR dataset, allowing for efficient downstream mineral identification. By processing raw spectra within the neural network model, our method substantially reduces the overall time required for preprocessing, while preserving and even enhancing the quality of spectral features essential for mineral classification. Using a standard system with an additional NVIDIA T1600 GPU, the proposed model reduces the preprocessing time of the same MTRDR scene to just 5 minutes.

Our objective in developing this model is to streamline hyperspectral data preprocessing on a large scale, facilitating real-time mineral mapping across Martian terrains. This objective aligns with the goals of planetary science, which aims to understand the surface composition of Mars, its geologic and climatic evolution, and any resources that might support human exploration. By achieving efficient and high-quality preprocessing of CRISM MTRDR hyperspectral data, the proposed model advances both the study of Martian geology and practical applications that could contribute to human missions on Mars.

Another challenge in Martian mineral identification is the limited availability of ground truth data for model training and validation. In Earth-based hyperspectral studies, field samples and lab analyses can be used as ground truth; however, in Martian studies, such data is sparse and inferred indirectly. Instead, researchers rely on spectral libraries—compilations of known spectral signatures for various minerals—for training and testing. The Mars-focused MICA spectral library, which includes reference spectra for minerals commonly found or expected on Mars, is the most widely used source for validating models by visually comparing test spectra to library samples. In this work, we address the lack of ground truth by developing synthetic spectra based on true spectra from the MICA library, augmented with fluctuations and baseline curvatures typical of MTRDR data. This augmentation strategy introduces variability that better represents real-world data, while preserving the characteristic absorption features critical for mineral identification.

The design of our UNet model incorporates several layers to achieve an efficient and scalable solution for hyperspectral preprocessing. The model architecture includes encoder and decoder blocks, each designed to handle one-dimensional spectral data by performing 1D convolution operations. The encoder blocks downsample the input spectral data, capturing important feature representations and reducing the data dimensionality to simplify processing. The decoder blocks, conversely, reconstruct the spectral data to the original resolution, enhancing specific mineralogical features and improving spectral clarity. Skip connections between encoder and decoder layers ensure that essential details are preserved during the data transformation, allowing the model to maintain a balance between feature abstraction and preservation. This architecture enables the model to retain vital information while efficiently preprocessing each spectrum, ultimately enhancing the quality and speed of mineral identification.

To validate the effectiveness of the proposed model, we evaluate its performance using a labeled set of Martian minerals curated by Plebani et al. These minerals were classified using a hierarchical Bayesian classifier and collected from multiple Martian locations. This labeled dataset serves as a reference for measuring the mineral identification accuracy of our model. In our evaluation, accuracy is defined by the match between the mineral labels identified by MICAnet, a mineral classification model, and those provided in the Plebani et al. dataset. Following preprocessing with our UNet-based autoencoder, the processed spectra are passed through MICAnet, which then performs mineral classification. By comparing the classification results with the reference labels, we assess the accuracy of our preprocessing model and its contribution to mineral identification on Mars.

The results of this study demonstrate that the proposed UNet-based model for spectral preprocessing significantly reduces the time required for data preparation while maintaining high classification accuracy. With a 5\% improvement in mineral identification accuracy and a processing time reduction of approximately 30\% compared to the traditional preprocessing pipeline, our approach presents a compelling solution for hyperspectral preprocessing. By eliminating the need for individual preprocessing steps, the model not only simplifies the data pipeline but also enables more efficient large-scale mineral mapping efforts. This capability is particularly valuable for planetary missions, where rapid data processing is essential for timely insights into surface composition and resource distribution.

% In summary, this paper introduces a UNet-based neural network model that preprocesses CRISM MTRDR hyperspectral data on the Martian surface, bypassing the traditional preprocessing pipeline. By integrating all preprocessing steps into a single, efficient model, the approach significantly improves the speed and quality of mineral identification, paving the way for large-scale, real-time spectral analysis on Mars. Through continued advancements in hyperspectral data processing, this research contributes to the broader objectives of Martian exploration and planetary science, supporting both scientific inquiry and potential future exploration efforts on Mars.
